A Probabilistic Perspective on Model Collapse

In recent years, model collapse has become a critical issue in language model training, making it essential to understand the underlying mechanisms driving this phenomenon. In this paper, we investigate recursive parametric model training from a probabilistic perspective, aiming to characterize the conditions under which model collapse occurs and, crucially, how it can be mitigated. We conceptualize the recursive training process as a random walk of the model estimate, highlighting how the sample size influences the step size and how the estimation procedure determines the direction and potential bias of the random walk. Under mild conditions, we rigorously show that progressively increasing the sample size at each training step is necessary to prevent model collapse. In particular, when the estimation is unbiased, the required growth rate follows a superlinear pattern. This rate needs to be accelerated even further in the presence of substantial estimation bias. Building on this probabilistic framework, we also investigate the probability that recursive training on synthetic data yields models that outperform those trained solely on real data. Moreover, we extend these results to general parametric model family in an asymptotic regime. Finally, we validate our theoretical results through extensive simulations and a real-world dataset.

==> Tmpe.tex <==
\begin{comment}
    
\textbf{Experiment.} To obtain a rough understanding of \textbf{Q1}-\textbf{Q3}, we conduct the following experiment of recursive Gaussian distribution estimation.
\begin{enumerate}
    \item We consider $N(\bm{\theta}^\star,\bm{I}_p)$ as the real distribution with $\bm{\theta}^\star$ being $p$-dimensional zero vector.
    \item During the recursive training, we estimate $\widehat{\bm{\theta}}_t = \frac{1}{n}\sum_{i=1}^n \bm{x}_{t-1,i}$ for $1 \leq T \leq 100$ and assume the covariance structure is known.
    \item We consider $(n,p) \in \{100,200\} \times \{2,4,6\}$ and report estimated $P_1(T) = \mathbb{P}(p^{-\frac{1}{2}}\|\widehat{\bm{\theta}}_T - \bm{\theta}^\star\|_2 \leq 0.5)$, $P_2(T) = \mathbb{P}(\Vert \widehat{\bm{\theta}}_T - \bm{\theta}^\star\|_2 < \|\widehat{\bm{\theta}}_1 - \bm{\theta}^\star\|_2)$, and $P_3(T) = \mathbb{P}(\cup_{t=1}^T\{\Vert \widehat{\bm{\theta}}_t - \bm{\theta}^\star\|_2 < \|\widehat{\bm{\theta}}_1 - \bm{\theta}^\star\|_2\})$ for cases $10 \leq T \leq 100$ in $2,000$ replications.
    \item Steps 1-3 are repeated 50 times for plotting the 95\% confidence intervals of estimated $P_1(T)$, $P_2(T)$, and $P_3(T)$.
\end{enumerate}

In this experiment, we aim to investigate how $(n, T, p)$ influences the values of $P_1(T)$, $P_2(T)$, and $P_3(T)$. Specifically, $P_1(T)$ denotes the probability that $\widehat{\bm{\theta}}_T$ remains close to the true parameter $\bm{\theta}^\star$, normalized by the data dimension. The quantity $P_2(T)$ reflects the probability that the final estimator $\widehat{\bm{\theta}}_T$ outperforms the baseline estimator $\widehat{\bm{\theta}}_1$, which is trained solely on real data. Meanwhile, $P_3(T)$ captures the probability that a better estimate than $\widehat{\bm{\theta}}_1$ appears at some point during the recursive training process. The simulation results are reported in Figure~\ref{Fig:Exp2}.





\begin{figure}[htbp]
  \centering
  \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{Exp2_100_0.png}
    \caption{$P_1(T): n=100$}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{Exp2_100_1.png}
    \caption{$P_2(T): n=100$}
        \label{fig2-temp1}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{Exp2_100_2.png}
    \caption{$P_3(T): n=100$}
        \label{fig2-temp11}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{Exp2_200_0.png}
    \caption{$P_1(T): n=200$}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{Exp2_200_1.png}
    \caption{$P_2(T): n=200$}
    \label{fig2-temp2}
  \end{subfigure}
  \begin{subfigure}[b]{0.3\textwidth}
    \includegraphics[width=\textwidth]{Exp2_200_2.png}
    \caption{$P_3(T): n=200$}
        \label{fig2-temp22}
  \end{subfigure}
  \caption{Estimated values of \( P_1(T), P_2(T) \), and \( P_3(T) \) with 95\% confidence intervals for \( 10 \leq T \leq 100 \), shown for \( n = 100 \) (top) and \( n = 200 \) (bottom).
}
\label{Fig:Exp2}
\end{figure}

As shown in Figure~\ref{Fig:Exp2}, $P_1(T)$ decreases as $T$ increases, suggesting that $\widehat{\bm{\theta}}_T$ is more likely to deviate from $\bm{\theta}^\star$ as the recursive training progresses. Additionally, when the sample size $n$ increases from 100 to 200, $P_1(T)$ increases consistently across all values of $p$. This is expected, as a larger sample size better preserves information about the underlying distribution, thereby mitigating the risk of model collapse. An interesting observation is that when $T$ is small, $P_1(T)$ tends to be larger for higher data dimensions $p$. However, as $T$ increases, $P_1(T)$ exhibits a more pronounced decline for larger $p$, indicating that higher dimensional models are more sensitive to recursive training and suffer greater degradation in estimation accuracy over time.


A similar pattern is observed for $P_2(T)$: it decreases as either $T$ or $p$ increases, indicating that obtaining a final model through recursive training that outperforms one trained purely on real data becomes increasingly rare as model complexity and the number of training steps increase. Interestingly, $P_2(T)$ appears to be unaffected by the sample size $n$, as evidenced by Figures~\ref{fig2-temp1} and~\ref{fig2-temp2}, which show nearly identical curves. Conversely, the probability of obtaining a model that outperforms the one trained on real data increases with $T$ and eventually converges to a value less than one. As model complexity $p$ increases, this probability tends to decrease. Furthermore, an interesting finding is that $P_3(T)$ also appears to be insensitive to the sample size $n$, as evidenced by the nearly identical results shown in Figures~\ref{fig2-temp11} and~\ref{fig2-temp22}.
\end{comment}

